The Challenge of Multi-Operand Adders in CNNs on FPGAs: How not to solve it!

Convolutional Neural Networks (CNNs) are computationally intensive algorithms that currently require dedicated hardware to be executed. In the case of FPGA-Based accelerators, we point-out in this work the challenge of Multi-Operand Adders (MOAs) and their high resource utilization in an FPGA implementation of a CNN. To address this challenge, two optimization strategies, that rely on time-multiplexing and approximate computing, are investigated. At first glance, the two strategies looked promising to reduce the footprint of a given architectural mapping, but when synthesized on the device, none of them gave the expected results. Experimental sections analyze the reasons of these unexpected results.

==> tikz/serial_moa.tex <==
\begin{tikzpicture}[scale=0.8, every node/.style={scale=0.9}]

    \tikzset{prod/.style={draw,circle,minimum size=0.5cm}}; 
    \tikzset{io/.style={}};
    
    \node [prod] (add0) at (4,-0.25) {$+$};
    \node [prod] (add1) at (4,-1.25) {$+$};
    \node (addd) at (4,-2.125) {$\vdots$};
    \node [prod] (add2) at (4,-4.25) {$+$};
    \node [prod] (add3) at (4,-3.25) {$+$};
    
    \node [prod] (add4) at (5,-0.75) {$+$};
    \node [prod] (add5) at (5,-3.75) {$+$};
    \node (addp) at (5,-2.25) {$\hdots$};
    
    \node [prod] (add6) at (6,-1.75) {$+$};
    \node [prod] (add7) at (6,-2.75) {$+$};
    \node [prod] (add8) at (7,-2.25) {$+$};
    
    
    \draw[->,>=latex] (add1)--(add4);
    \draw[->,>=latex] (add0)--(add4);
    \draw[->,>=latex] (add2)--(add5);
    \draw[->,>=latex] (add3)--(add5);
    \draw[->,>=latex] (add6)--(add8);
    \draw[->,>=latex] (add7)--(add8);
    
    
    %\draw[thick,dotted] (3,1) rectangle (7.5,-5.25);
    
    
\end{tikzpicture}
